Data-dependent Sample Complexity of Deep Neural Networks via Lipschitz Augmentation

Existing Rademacher complexity bounds for neural networks rely only on norm control of the weight matrices and depend exponentially on depth via a product of the matrix norms. Lower bounds show that this exponential dependence on depth is unavoidable when no additional properties of the training data are considered. We suspect that this conundrum comes from the fact that these bounds depend on the training data only through the margin. In practice, many data-dependent techniques such as Batchnorm improve the generalization performance. For feedforward neural nets as well as RNNs, we obtain tighter Rademacher complexity bounds by considering additional data-dependent properties of the network: the norms of the hidden layers of the network, and the norms of the Jacobians of each layer with respect to all previous layers. Our bounds scale polynomially in depth when these empirical quantities are small, as is usually the case in practice. To obtain these bounds, we develop general tools for augmenting a sequence of functions to make their composition Lipschitz and then covering the augmented functions. Inspired by our theory, we directly regularize the network's Jacobians during training and empirically demonstrate that this improves test performance.

==> cover_8pages.tex <==






==> covering.tex <==






==> macro.tex <==


\usepackage{amsthm}

\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{fullpage}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}

\usepackage{bbm}
\usepackage{dsfont}
\usepackage{graphicx}
\usepackage{natbib}
\usepackage{cases}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true, allcolors=blue]{hyperref}


\def\shownotes{1}  \ifnum\shownotes=1
\newcommand{\authnote}[2]{$\ll$\textsf{\footnotesize #1 notes: #2}$\gg$}
\newcommand{\Tnote}[1]{{\color{blue}\authnote{Tengyu}{#1}}}
\newcommand{\Cnote}[1]{{\color{red}\authnote{Colin}{#1}}}
\newcommand{\jnote}[1]{{\color{red}\authnote{Jason}{#1}}}


\newtheorem{proposition}{Proposition}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{example}{Example}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{claim}{Claim}[section]


\newcommand{\genparam}{\Theta}
\newcommand{\bgenparam}{\bar{\Theta}}
\newcommand{\param}{\theta}
\newcommand{\bparam}{\bar{\theta}}
\newcommand{\hparam}{\hat{\theta}}
\newcommand{\ones}{\vec{1}}
\newcommand{\zeros}{\vec{0}}
\newcommand{\diag}{\text{diag}}
\newcommand{\TODO}[1]{{\color{blue}[TODO: {#1}]}}
\newcommand{\subj}{\textup{subject to }}
\newcommand{\bdir}{\bparam}
\newcommand{\hdir}{\hat{u}}
\newcommand{\dir}{u}
\newcommand{\weight}{w}
\newcommand{\sph}{\sphd}
\newcommand{\sphd}{\mathbb{S}^d}
\newcommand{\sign}{\textup{sign}}
\newcommand{\supp}{\text{supp}}
\newcommand{\hyp}{\mathcal{H}}
\newcommand{\radub}{R}
\newcommand{\E}{\mathbb{E}}
\newcommand{\betarv}{\bm{\beta}}
\newcommand{\yrv}{\bm{y}}
\newcommand{\tr}{\textup{tr}}
\newcommand{\vol}{\text{Vol}}
\newcommand{\dist}{\rho}
\newcommand{\R}{\mathbb{R}}
\newcommand{\1}{\mathbbm{1}}
\newcommand{\argmax}{\arg \max}
\newcommand{\bart}{\bar{t}}
\newcommand{\id}{I}




\newtheorem*{remark*}{Remark}
\newtheorem{observation}[theorem]{Observation}
\newtheorem*{observation*}{Observation}

\numberwithin{equation}{section}


\newcommand{\yrvu}{\bm{Y}}


\newcommand{\spaceone}{\mathcal{L}^1}
\newcommand{\spacetwo}{\mathcal{L}^2}
\newcommand{\spaceinf}{\mathcal{L}^{\infty}}
\newcommand{\spacep}{\mathcal{P}}
\newcommand{\poly}{\textup{poly}}

\newcommand{\Gnorm}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
		\right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}
	
	\newcommand{\gnorm}[1]{{\vert\kern-0.25ex\vert\kern-0.25ex\vert #1 
\vert\kern-0.25ex\vert\kern-0.25ex\vert}}






==> macro_colt.tex <==






\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{multirow}
\usepackage[export]{adjustbox}
\usepackage{amsmath,amssymb,amsthm}
\usepackage{hyperref}
\usepackage{bbm}
\usepackage{dsfont}
\usepackage{graphicx}
\usepackage{natbib}
\usepackage{cases}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage{wrapfig}



\def\shownotes{1}  \ifnum\shownotes=1
\newcommand{\authnote}[2]{$\ll$\textsf{\footnotesize #1 notes: #2}$\gg$}
\else
\newcommand{\authnote}[2]{}
\fi
\newcommand{\Tnote}[1]{{\color{blue}\authnote{Tengyu}{#1}}}
\newcommand{\Cnote}[1]{{\color{red}\authnote{Colin}{#1}}}
\newcommand{\jnote}[1]{{\color{red}\authnote{Jason}{#1}}}

\newtheorem{proposition}{Proposition}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{claim}[theorem]{Claim}


\newcommand{\genparam}{\Theta}
\newcommand{\bgenparam}{\bar{\Theta}}
\newcommand{\param}{\theta}
\newcommand{\bparam}{\bar{\theta}}
\newcommand{\hparam}{\hat{\theta}}
\newcommand{\ones}{\vec{1}}
\newcommand{\zeros}{\vec{0}}
\newcommand{\diag}{\text{diag}}
\newcommand{\TODO}[1]{{\color{blue}[TODO: {#1}]}}
\newcommand{\subj}{\textup{subject to }}
\newcommand{\bdir}{\bparam}
\newcommand{\hdir}{\hat{u}}
\newcommand{\dir}{u}
\newcommand{\weight}{w}
\newcommand{\sph}{\sphd}
\newcommand{\sphd}{\mathbb{S}^d}
\newcommand{\sign}{\textup{sign}}
\newcommand{\supp}{\text{supp}}
\newcommand{\hyp}{\mathcal{H}}
\newcommand{\radub}{R}
\newcommand{\E}{\mathbb{E}}
\newcommand{\betarv}{\bm{\beta}}
\newcommand{\yrv}{\bm{y}}
\newcommand{\tr}{\textup{tr}}
\newcommand{\vol}{\text{Vol}}
\newcommand{\dist}{\rho}
\newcommand{\R}{\mathbb{R}}
\newcommand{\1}{\mathbbm{1}}
\newcommand{\argmax}{\arg \max}
\newcommand{\bart}{\bar{t}}
\newcommand{\id}{I}








\newcommand{\yrvu}{\bm{Y}}


\newcommand{\spaceone}{\mathcal{L}^1}
\newcommand{\spacetwo}{\mathcal{L}^2}
\newcommand{\spaceinf}{\mathcal{L}^{\infty}}
\newcommand{\spacep}{\mathcal{P}}
\newcommand{\poly}{\textup{poly}}

\newcommand{\Gnorm}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
		\right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}
	
	\newcommand{\gnorm}[1]{{\vert\kern-0.25ex\vert\kern-0.25ex\vert #1 
\vert\kern-0.25ex\vert\kern-0.25ex\vert}}






==> notations.tex <==




\section{Notation}\label{sec:notations}

\Tnote{let's check whether we need all of these notations for the first 8 pages. We can have another section or subsecton for notations in appendix. This saves some space.. }
Let $\one(E)$ be the indicator function of event $E$. Let $l_{\textup{0-1}}$ denote the standard 0-1 loss. For $\kappa\ge 0$, Let $\one[\le \kappa](\cdot)$ be the softened indicator function defined as 
\begin{align}
\one[\le \kappa](t) =  \left\{\begin{array}{ll}
1 & \textup{ if } t \le \kappa \\
2 - t/\kappa & \textup{ if } \kappa \le t \le 2\kappa \\
0 & \textup{ if } 2\kappa \le t  \\
\end{array}\right.\nonumber
\end{align}
Note that $\one[\le \kappa]$ is $\kappa^{-1}$-Lipschitz. Define the norm $\| \cdot \|_{p, q}$ by $\|A\|_{p, q} \triangleq \Big(\sum_{j} \big(\sum_i A_{i, j}^p \big)^{q/p}\Big)^{1/q}$.
Let $P_n$ be a uniform distribution over $n$ points $\{x_1,\dots, x_n\}\subset \cD_x$. Let $f$ be a function that maps $\cD_x$ to some output space $\cD_f$, and assume both spaces are equipped with some norms $\gnorm{\cdot}$ (these norms can be different but we use the same notations for them). Then the $L_2(P_n, \gnorm{\cdot})$ norm of the function $f$ is defined as 
$
\|f\|_{L_2(P_n, \gnorm{\cdot})} \triangleq  \left(\frac{1}{n} \sum_i \gnorm{f(x_i)}^2\right)^{1/2}
$.
We use $D$ to denote total derivative operator, and thus $Df(x)$ represents the Jacobian of $f$ at $x$.


Suppose $\cF$ is a family of functions from $\cD_x$ to $\cD_f$. 
Let $\mathcal{C}(\epsilon, \mathcal{F}, \rho)$ be the covering number of the function class $\cF$ w.r.t. metric $\rho$ with cover size $\epsilon$. 
In many cases, the covering number depends on the examples through the norms of the examples, and in this paper we only work with these cases. 
Thus, we let $\cover(\epsilon,\mathcal{F}, s)$ be the maximum covering number for any possible $n$ data points with norm not larger than $s$. 
Precisely, if we define $\mathcal{P}_{n,s}$ to be the set of all possible uniform distributions supported on $n$ data points with norms not larger than $s$, then 
\begin{align*}
\cover(\epsilon, \mathcal{F}, s) \triangleq \sup_{P_n \in \mathcal{P}_{n,s}} \mathcal{C}(\epsilon, \mathcal{F}, L_2(P_n, \gnorm{\cdot}))
\end{align*}
Suppose $\mathcal{F}$ contains functions with $m$ inputs that map from a tensor product $m$ Euclidean space to Euclidean space, then we define 
$
\cover(\epsilon, \mathcal{F}, (s_1,\dots, s_m)) \triangleq \sup_{\substack{P: \forall (x_1,\dots, x_m) \in \supp(P)\\ \|x_i\|\le s_i}} \mathcal{C}(\epsilon, \mathcal{F}, L_2(P))
$.








==> old_notes.tex <==
\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\
\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\								


